Complexity of the path avoiding forbidden pairs problem revisited

Let G = (V, E) be a directed acyclic graph with two distinguished vertices s, t and let F be a set of forbidden pairs of vertices. We say that a path in G is safe, if it contains at most one vertex from each pair {u, v} in F. Given G and F, the path avoiding forbidden pairs (PAFP) problem is to find a safe s-t path in G. We systematically study the complexity of different special cases of the PAFP problem defined according to the mutual positions of forbidden pairs. Fix one topological ordering of vertices; we say that pairs {u, v} and {x, y} are disjoint, if u, v < x, y, nested, if u < x, y < v, and halving, if u < x < v < y. The PAFP problem is known to be NP-hard in general or if no two pairs are disjoint; we prove that it remains NP-hard even when no two forbidden pairs are nested. On the other hand, if no two pairs are halving, the problem is known to be solvable in cubic time. We simplify and improve this result by showing an O(M(n)) time algorithm, where M(n) is the time to multiply two n \times n boolean matrices.

==> Makefile <==
all: main.pdf

clean:
	-rm main.aux main.bbl main.blg main.log main.log main.lot main.out \
	main.dvi main.ps main.pdf *~
	make -C figures clean

main.ps: main.dvi
	dvips main -o main.ps

main.pdf: main.tex *.tex *.bib figs/*
	pdflatex main
	pdflatex main
	-bibtex main
	pdflatex main
	pdflatex main


main.dvi: figures main.tex *.tex *.bib
	latex main
	latex main
	-bibtex main
	latex main
	latex main

.PHONY: figures all bib

figures:
	make -C figures

